A thermodynamically consistent theory of stress-gradient plasticity

As an extension to strain-gradient models of size-dependent plastic behaviour, this work proposes a model for a stress-gradient theory. The model is distinguished from earlier works on the topic by its being embedded in a thermodynamically consistent framework. The development is carried out in the context of single-crystal plasticity, and draws on thermodynamically consistent models for single-crystal conventional and strain-gradient plasticity. The model is explored numerically using the example of torsion of a thin wire comprising a face centred cubic crystal, and its behaviour compared with that based on a recent disequilibrium density model of size-dependent plasticity.

==> tikzPics/AK_Unitcell.tex <==
\newcommand{\background}{
 \coordinate (A0) at (0,0,0);
    \coordinate (A1) at (1,0,0);
    \coordinate (A2) at (0,1,0);
    \coordinate (A3) at (0,0,1);

    \coordinate (A4) at (1,1,0);
    \coordinate (A5) at (1,0,1);
    \coordinate (A6) at (0,1,1);
    \coordinate (A7) at (1,1,1);

    \coordinate (A8) at (0.5,0.5,0);
    \coordinate (A9) at (0.5,0,0.5);
    \coordinate (A10) at (0,0.5,0.5);

    \coordinate (A11) at (0.5,0.5,1);
    \coordinate (A12) at (0.5,1,0.5);
    \coordinate (A13) at (1,0.5,0.5);

    \draw[black!25, dashed] (A0) -- (A8) -- (A4);
    \draw[black!25, dashed] (A0) -- (A10) -- (A6);
    \draw[black!25, dashed] (A1) -- (A8) -- (A2);
    \draw[black!25, dashed] (A2) -- (A10) -- (A3);
    \draw[black!25, dashed] (A5) -- (A9) -- (A0);
    \draw[black!25, dashed] (A3) -- (A9) -- (A1);
    \draw[black!25] (A0) -- (A1);
    \draw[black!25] (A0) -- (A2);
    \draw[black!25] (A0) -- (A3);
    \fill[blue!25] (A0) circle (1pt);
    \fill[blue!25] (A8) circle (1pt);
    \fill[blue!25] (A10) circle (1pt);
    \fill[blue!25] (A9) circle (1pt);  
}

\newcommand{\foreground}{
    \coordinate (A0) at (0,0,0);
    \coordinate (A1) at (1,0,0);
    \coordinate (A2) at (0,1,0);
    \coordinate (A3) at (0,0,1);

    \coordinate (A4) at (1,1,0);
    \coordinate (A5) at (1,0,1);
    \coordinate (A6) at (0,1,1);
    \coordinate (A7) at (1,1,1);

    \coordinate (A8) at (0.5,0.5,0);
    \coordinate (A9) at (0.5,0,0.5);
    \coordinate (A10) at (0,0.5,0.5);

    \coordinate (A11) at (0.5,0.5,1);
    \coordinate (A12) at (0.5,1,0.5);
    \coordinate (A13) at (1,0.5,0.5);
    
       
    \draw[black, dashed] (A1) -- (A13) -- (A7);
    \draw[black, dashed] (A3) -- (A11) -- (A7);
    \draw[black, dashed] (A5) -- (A13) -- (A4);
    \draw[black, dashed] (A6) -- (A11) -- (A5);
    \draw[black, dashed] (A7) -- (A12) -- (A2);
    \draw[black, dashed] (A4) -- (A12) -- (A6);
    \draw[black] (A3) -- (A5);
    \draw[black] (A3) -- (A6);
    \draw[black] (A6) -- (A2);
    \draw[black] (A5) -- (A1);
    \draw[black] (A7) -- (A4);
    \draw[black] (A5) -- (A7);
    \draw[black] (A1) -- (A4);
    \draw[black] (A6) -- (A7);
    \draw[black] (A2) -- (A4);    
}

\newcommand{\atoms}{
    \coordinate (A0) at (0,0,0);
    \coordinate (A1) at (1,0,0);
    \coordinate (A2) at (0,1,0);
    \coordinate (A3) at (0,0,1);

    \coordinate (A4) at (1,1,0);
    \coordinate (A5) at (1,0,1);
    \coordinate (A6) at (0,1,1);
    \coordinate (A7) at (1,1,1);

    \coordinate (A8) at (0.5,0.5,0);
    \coordinate (A9) at (0.5,0,0.5);
    \coordinate (A10) at (0,0.5,0.5);

    \coordinate (A11) at (0.5,0.5,1);
    \coordinate (A12) at (0.5,1,0.5);
    \coordinate (A13) at (1,0.5,0.5);
    
       

    \fill[blue] (A3) circle (1pt);
    \fill[blue] (A4) circle (1pt);
    \fill[blue] (A5) circle (1pt);
    \fill[blue] (A6) circle (1pt);
    \fill[blue] (A7) circle (1pt);
    \fill[blue] (A11) circle (1pt);
    \fill[blue] (A12) circle (1pt);
    \fill[blue] (A13) circle (1pt);
    \fill[blue] (A1) circle (1pt);
    \fill[blue] (A2) circle (1pt); 
}
\newcommand{\cosyCircle}{
    \begin{scope}[zyplane = 0]
    	\fill[yellow!15] (0.5,0.5) circle (1/1.41);
    	\filldraw[fill=yellow](1,1) -- (1,0)
    	arc[start angle = -45, end angle = 45, radius=1/1.41] -- cycle;
    	\filldraw[fill=yellow](0,1) -- (1,1)
    	arc[start angle = 45, end angle = 135, radius=1/1.41] -- cycle;
    	\draw[black!25] (0.5,0.5) circle (1/1.41);
    	\draw[black!50] (0.5,0.5) -- (1,0.5);
    	\draw[black!50] (0.5,0.5) -- (0.5,1);
    	\draw[black, ->] (1,0.5) -- (1.5,0.5) node[anchor=south, black]{\footnotesize z};
    	\draw[black, ->] (0.5,1) -- (0.5,1.5) node[anchor=south, black]{\footnotesize y};
    \end{scope}
    }


\tdplotsetmaincoords{68}{110}
\begin{tikzpicture}[
  tdplot_main_coords
  ]  

	\tikzset{zyplane/.style={canvas is zy plane at x=#1,very thin}}
  
    \coordinate (A0) at (0,0,0);
    \coordinate (A1) at (1,0,0);
    \coordinate (A2) at (0,1,0);
    \coordinate (A3) at (0,0,1);

    \coordinate (A4) at (1,1,0);
    \coordinate (A5) at (1,0,1);
    \coordinate (A6) at (0,1,1);
    \coordinate (A7) at (1,1,1);

    \coordinate (A8) at (0.5,0.5,0);
    \coordinate (A9) at (0.5,0,0.5);
    \coordinate (A10) at (0,0.5,0.5);

    \coordinate (A11) at (0.5,0.5,1);
    \coordinate (A12) at (0.5,1,0.5);
    \coordinate (A13) at (1,0.5,0.5);
    
    \begin{scope}[scale = 1.35]
    
 	\begin{scope}[shift={(0,0,0)}]
 	\cosyCircle
    \background
    \foreground    
    \fill[green, opacity=0.25] (A1) -- (A2) -- (A3); % 1,2,3
	\draw[red, ->] (A3) -- ($(A3)!1.2!(A2)$) node[anchor=west, black]{\footnotesize 1};
	\draw[red, ->] (A3) -- ($(A3)!1.2!(A1)$) node[anchor=north, black]{\footnotesize 2};
	\draw[red, ->] (A2) -- ($(A2)!1.2!(A1)$) node[anchor=east, black]{\footnotesize 3};
 	\atoms 	
 	\end{scope}
 
    
    
 	\begin{scope}[shift={(-0.726,2,0)}]
 	\cosyCircle
    \background
    \foreground
    \fill[green, opacity=0.25] (A2) -- (A3) -- (A7); % 4,5,6
	\draw[red, ->] (A3) -- ($(A3)!1.2!(A2)$) node[anchor=west, black]{\footnotesize 4};
	\draw[red, ->] (A2) -- ($(A2)!1.6!(A7)$) node[anchor=south, black]{\footnotesize 5};
	\draw[red, ->] (A7) -- ($(A7)!1.4!(A3)$) node[anchor=east, black]{\footnotesize 6};	
 	\atoms 	
 	\end{scope}
 
    
    
 	\begin{scope}[shift={(-1.452,4,0)}]
 	\cosyCircle
    \background
    \foreground
    \fill[green, opacity=0.25] (A1) -- (A3) -- (A7); % 7,8,9
	\draw[red, ->] (A1) -- ($(A1)!1.5!(A7)$) node[anchor=west, black]{\footnotesize 7};
	\draw[red, ->] (A3) -- ($(A3)!1.2!(A1)$) node[anchor=north, black]{\footnotesize 8};
	\draw[red, ->] (A7) -- ($(A7)!1.2!(A3)$) node[anchor=south, black]{\footnotesize 9};	
 	\atoms 	
 	\end{scope}
 
    
    
 	\begin{scope}[shift={(-2.178,6,0)}]
 	\cosyCircle
    \background
    \foreground
    \fill[green, opacity=0.25] (A1) -- (A2) -- (A7); % 10,11,12
 	\draw[red, ->] (A1) -- ($(A1)!1.5!(A7)$) node[anchor=west, black]{\footnotesize 10};
 	\draw[red, ->] (A1) -- ($(A1)!1.2!(A2)$) node[anchor=west, black]{\footnotesize 11};
 	\draw[red, ->] (A2) -- ($(A2)!2.0!(A7)$) node[anchor=south, black]{\footnotesize 12}; 	
 	\atoms 	
 	\end{scope}
 	
 	
 	\end{scope}
 
\end{tikzpicture}

==> tikzPics/AK_diff_l_r.tex <==
\begin{tikzpicture}
%pgfplotsset{
%tick label style = {font=\sansmath\sffamily, /pgf/number format/.cd,
%        fixed},
%  every axis label = {font=\sansmath\sffamily},
%  legend style = {font=\sansmath\sffamily},
%  label style = {font=\sansmath\sffamily}
%}
\begin{axis}[%
 x tick label style={
        /pgf/number format/.cd,
            fixed,
            precision=3,
        /tikz/.cd
    },
width=6cm,
height=5cm,
scale only axis,
separate axis lines,
scaled x ticks = false,
scaled y ticks = false,
xmin=0,
xmax=5,
ymin=0000,
ymax=240,
%ymin=900,
%ymax=1200,
%xtick={0,0.01,0.02},
%ytick={1000,1200},
%axis background/.style={fill=white},
%title style={align=center},
ylabel={Torque in \si{\nano\newton\meter}},
xlabel={Twist $\kappa$ in \si{\per\milli\meter}},
%%title={Tanh, microhard},
legend pos = south east,
legend cell align={left}
%legend style={at={(0.005,0.2)},anchor=south west}
]

\input{tikzPics/AK_diff_l_r_data.tex}

\end{axis}
\end{tikzpicture}%

==> tikzPics/AK_diff_l_r_data.tex <==
\addplot[color=blue,
mark = none,
]
table[x expr={\thisrow{a}*200}, y expr={\thisrow{b}/1000}, col sep=space, row sep=newline]{
a b
0.000000 0.000000
0.000833 37180.500000
0.001667 74367.200000
0.002500 111522.000000
0.003333 146097.000000
0.004167 170405.000000
0.005000 184084.000000
0.005833 191369.000000
0.006667 195385.000000
0.007500 197733.000000
0.008333 199188.000000
0.009167 200135.000000
0.010000 200779.000000
0.010833 201232.000000
0.011667 201562.000000
0.012500 201810.000000
0.013333 202000.000000
0.014167 202149.000000
0.015000 202268.000000
0.015833 202365.000000
0.016667 202446.000000
0.017500 202515.000000
0.018333 202573.000000
0.019167 202624.000000
0.020000 202669.000000
0.020833 202709.000000
0.021667 202745.000000
0.022500 202778.000000
0.023333 202809.000000
0.024167 202837.000000
0.025000 202863.000000
};
\addlegendentry{$\ell = 0.00$};



%
\addplot[color=black,
mark = none,
]
table[x expr={\thisrow{a}*200}, y expr={\thisrow{b}/1000}, col sep=space, row sep=newline]{
a b 
0.000000 0.000000
0.000833 37180.500000
0.001667 74367.200000
0.002500 111528.000000
0.003333 146512.000000
0.004167 172099.000000
0.005000 187182.000000
0.005833 195466.000000
0.006667 200122.000000
0.007500 202891.000000
0.008333 204635.000000
0.009167 205792.000000
0.010000 206593.000000
0.010833 207167.000000
0.011667 207592.000000
0.012500 207916.000000
0.013333 208169.000000
0.014167 208370.000000
0.015000 208534.000000
0.015833 208670.000000
0.016667 208784.000000
0.017500 208882.000000
0.018333 208966.000000
0.019167 209041.000000
0.020000 209107.000000
0.020833 209166.000000
0.021667 209219.000000
0.022500 209268.000000
0.023333 209313.000000
0.024167 209355.000000
0.025000 209394.000000
};
\addlegendentry{{$\ell = 0.05$ $q=0$}};


%
\addplot[color=black, dashed,
mark = none
]
table[x expr={\thisrow{a}*200}, y expr={\thisrow{b}/1000}, col sep=space, row sep=newline]{
a b 
0.000000 0.000000
0.000833 37180.500000
0.001667 74367.200000
0.002500 111530.000000
0.003333 146619.000000
0.004167 172561.000000
0.005000 188063.000000
0.005833 196658.000000
0.006667 201515.000000
0.007500 204415.000000
0.008333 206251.000000
0.009167 207475.000000
0.010000 208326.000000
0.010833 208940.000000
0.011667 209397.000000
0.012500 209747.000000
0.013333 210021.000000
0.014167 210241.000000
0.015000 210420.000000
0.015833 210570.000000
0.016667 210696.000000
0.017500 210805.000000
0.018333 210899.000000
0.019167 210982.000000
0.020000 211056.000000
0.020833 211123.000000
0.021667 211183.000000
0.022500 211239.000000
0.023333 211291.000000
0.024167 211338.000000
0.025000 211383.000000
};
\addlegendentry{ {$\ell = 0.05$ $q=1.4$}};


%
\addplot[color=red,
mark = none
]
table[x expr={\thisrow{a}*200}, y expr={\thisrow{b}/1000}, col sep=space, row sep=newline]{
a b 
0.000000 0.000000
0.000833 37180.500000
0.001667 74367.200000
0.002500 111534.000000
0.003333 146875.000000
0.004167 173675.000000
0.005000 190182.000000
0.005833 199511.000000
0.006667 204824.000000
0.007500 208018.000000
0.008333 210056.000000
0.009167 211425.000000
0.010000 212387.000000
0.010833 213087.000000
0.011667 213613.000000
0.012500 214018.000000
0.013333 214337.000000
0.014167 214594.000000
0.015000 214806.000000
0.015833 214984.000000
0.016667 215134.000000
0.017500 215264.000000
0.018333 215380.000000
0.019167 215480.000000
0.020000 215569.000000
0.020833 215650.000000
0.021667 215724.000000
0.022500 215792.000000
0.023333 215855.000000
0.024167 215913.000000
0.025000 215967.000000
};
\addlegendentry{ {$\ell = 0.10$ $q=0$}};


\addplot[color=red, dashed,
mark = none
]
table[x expr={\thisrow{a}*200}, y expr={\thisrow{b}/1000}, col sep=space, row sep=newline]{
a b 
0.000000 0.000000
0.000833 37180.500000
0.001667 74367.200000
0.002500 111536.000000
0.003333 147058.000000
0.004167 174523.000000
0.005000 191883.000000
0.005833 201874.000000
0.006667 207605.000000
0.007500 211078.000000
0.008333 213316.000000
0.009167 214835.000000
0.010000 215911.000000
0.010833 216700.000000
0.011667 217295.000000
0.012500 217762.000000
0.013333 218131.000000
0.014167 218431.000000
0.015000 218680.000000
0.015833 218893.000000
0.016667 219075.000000
0.017500 219233.000000
0.018333 219371.000000
0.019167 219499.000000
0.020000 219610.000000
0.020833 219717.000000
0.021667 219812.000000
0.022500 219897.000000
0.023333 219980.000000
0.024167 220056.000000
0.025000 220129.000000
};
\addlegendentry{ $\ell = 0.10$ $q=1.4$};

% example from our JMPS paper with disequillibrium densities
\addplot[color=green!50!black, solid,
mark = none
]
table[x expr={\thisrow{a}*200}, y expr={\thisrow{b}/1000}, col sep=space, row sep=newline]{
a b
0.000000 0.000000
0.000833 37180.500000
0.001667 74367.200000
0.002500 111522.000000
0.003333 146097.000000
0.004167 170408.000000
0.005000 184115.000000
0.005833 191468.000000
0.006667 195595.000000
0.007500 198078.000000
0.008333 199672.000000
0.009167 200733.000000
0.010000 201505.000000
0.010833 202108.000000
0.011667 202597.000000
0.012500 203045.000000
0.013333 203439.000000
0.014167 203805.000000
0.015000 204147.000000
0.015833 204474.000000
0.016667 204799.000000
0.017500 205128.000000
0.018333 205467.000000
0.019167 205817.000000
0.020000 206191.000000
0.020833 206590.000000
0.021667 207006.000000
0.022500 207443.000000
0.023333 207881.000000
0.024167 208353.000000
0.025000 208849.000000
};
\addlegendentry{ {DE densities \cite{Steinmann_etal2019}}};

==> tikzPics/AK_diff_l_r_zoom.tex <==
\begin{tikzpicture}
%pgfplotsset{
%tick label style = {font=\sansmath\sffamily, /pgf/number format/.cd,
%        fixed},
%  every axis label = {font=\sansmath\sffamily},
%  legend style = {font=\sansmath\sffamily},
%  label style = {font=\sansmath\sffamily}
%}
\begin{axis}[%
 x tick label style={
        /pgf/number format/.cd,
            fixed,
            precision=3,
        /tikz/.cd
    },
width=6cm,
height=5cm,
scale only axis,
separate axis lines,
scaled x ticks = false,
scaled y ticks = false,
xmin=0.7,
xmax=5,
ymin=150,
ymax=225,
%ymin=900,
%ymax=1200,
%xtick={0,0.01,0.02},
%ytick={1000,1200},
%axis background/.style={fill=white},
%title style={align=center},
ylabel={Torque in \si{\nano\newton\meter}},
xlabel={Twist $\kappa$ in \si{\per\milli\meter}},
%%title={Tanh, microhard},
legend pos = south east,
legend cell align={left}
%legend style={at={(0.005,0.2)},anchor=south west}
]

\input{tikzPics/AK_diff_l_r_data.tex}

\end{axis}
\end{tikzpicture}%
